Answering Ambiguous Questions with a Database of Questions, Answers, and Revisions

Many open-domain questions are under-specified and thus have multiple possible answers, each of which is correct under a different interpretation of the question. Answering such ambiguous questions is challenging, as it requires retrieving and then reasoning about diverse information from multiple passages. We present a new state-of-the-art for answering ambiguous questions that exploits a database of unambiguous questions generated from Wikipedia. On the challenging ASQA benchmark, which requires generating long-form answers that summarize the multiple answers to an ambiguous question, our method improves performance by 15% (relative improvement) on recall measures and 10% on measures which evaluate disambiguating questions from predicted outputs. Retrieving from the database of generated questions also gives large improvements in diverse passage retrieval (by matching user questions q to passages p indirectly, via questions q' generated from p).

==> 100_model_ambigqa.tex <==


\subsubsection{Question Revision}

In the next ablation experiment, we investigate whether the additional information retrieved from \database{} help differentiating answers. Here, we study a question revision sub-task using auxiliary information provided in ASQA dataset, in which each answer is paired with a revised question and a passage that contains the additional information used for the revision.


In the first experiment, we would like to use \database{} on a question revision task on AmbigQA \cite{min2020ambigqa}. The task is similar to extracting conditions when constructing \database{} (\S \ref{sec:cond_gen}), except that the additional information added to the revised question should be contrastive, i.e. it should differentiate its answer with others possible answers to the ambiguous questions. For example, to differentiate the answer ``the Michigan Stadium'' and ``Crisler Center'', one should provide the additional information ``\textit{basketball team}'' vs. ``\textit{football team}'', but not ``\textit{men's}'' vs. ``\textit{women's}''. 

A naive method to solve this task is to retrieve the most similar question and answer pairs from \database{} and directly returned their conditions (already represented as revised questions) as outputs. This method is sub-optimal, because any text spans, contrastive or not, could be used as conditions in \database{}. In fact, it is not possible for models to tell whether a condition is contrastive without knowing conditions for other answers. 

\subsubsection{Task} \label{sec:ambigqa_task}
In the question revision task, the model takes an ambiguous question $q$, a passage $p$, and an answer $a_i$ that exists in the passage, and it outputs a revised question $\tilde{q}$ such that $a_i$ is the unique answer to $\tilde{q}$.

% \textbf{Comparison to Conditions in \database{}.} The question revision task in AmbigQA is similar to generating conditions in the construction of \database{}, except that conditions generated in \database{} does not have to be contrastive. For example, ``men's'' is a valid condition in \database{} but cannot be used to differentiate answers. A baseline is to simply take retrieved answers as  


Previous models \hs{cite} simply takes the question $q$ and passage $p$ as input and train a seq-to-seq to directly generate the revised question $\tilde{q}$. Such methods are sub-optimal because the task requires models to aggregate multiple pieces of information for different answers which commonly spread across several passages. With the lack of necessary information, a commonly observed error is to simply pick any text spans, e.g. dates and locations, from passages and add them to the revised questions. 
% Even though the added information comes from the passages, it may not differentiate the answers.

The quality of revision is measured by a new metric, ``EDIT-F1'', proposed by \citep{min2020ambigqa} as the official evaluation metric in AmbigQA. Traditional metrics for sequence prediction, such as ROUGE and BLEU, are not appropriate in evaluating revised questions, because simply copying the original questions will already get high scores. In particular, predicting the original question without any revision leads to \hs{num} in ROUGE and \hs{num} in BLEU. The proposed ``EDIT-F1'' metric resolves this problem by only measuring \textit{edits}. For example, if the expected revision is ``Where is the home stadium of the Michigan Wolverines \{$+$ men's\} \{$+$ football\}'' which has edits ``$+$ men's'' and ``$+$ football'', while the prediction is ``Where is the home stadium of the Michigan Wolverines \{$+$ since\} \{$+$ 1967\}'', the EDIT-F1 is 0 even though the prediction matches the first few tokens of the reference.


\subsubsection{Method} \label{sec:ambigqa_method}
We propose to retrieve similar questions $q'$ with their answers and conditions, i.e. $\{(a_i, c_i)\}$, from \database{}, and augment the passage $p$ with retrieved information from answers and conditions. The retrieved answers and conditions $\{(a_i, c_i)\}$ provide background knowledge for models to determine what information can differentiate the answers. For example, the answer ``Crisler Center'' to the question above with conditions ``men's'' and ``basketball team'' suggests two potential ways to differentiate it with the other answer ``the Michigan Stadium''. Models can compare retrieved information with information from the provided passage, e.g. ``men's'' vs. ``women's'' or ``basketball'' vs. ``football'', to decide what information to use to revise the question.

% \subsubsection{Question Retrieval from \database{}}
% We propose to retrieve from \database{} to provide additional information for models to improve the performance of question revision. Questions, answers, and conditions retrieved from \database{} provide background knowledge for models to determine what information can differentiate the answers. For example, the answer ``Crisler Center'' to the question above with conditions expressed as a revised question ``Where is the home stadium of Michigan Wolverine men's basketball team?'' suggests ``men's'' and ``basketball team'' are two potential ways to differentiate it with the other answer ``the Michigan Stadium''. Models can compare retrieved information with information from the provided passage to determine how to revise the question.

% Retrieving questions from \database{} is similar to retrieving passages from text corpus. Upon retrieval, we treat the original ambiguous questions as queries, questions in \database{} as keys, and answers and conditions (represented as revised questions) as values. The retriever finds the most similar questions from \database{} and return their answers and conditions. We simply apply one of the state-of-the-art dense retrieval model, GTR \cite{ni2021large}, as our retriever to retrieve the top $k$ similar questions from \database{}.\footnote{We re-use GTR's checkpoint finetuned on NQ \cite{kwiatkowski2019natural} for our retrieval task. Note that GTR is trained for passage retrieval, but it is also applicable to our retrieval task since query encoder and passage encoder in GTR share same parameters.} GTR is similar to DPR except that it is pretrained on web-mined questions and corpus.

% \subsubsection{Question Revision}
We follow previous work \hs{cite} to finetune a T5 model to perform the question revision task. However, we augment the provided passage $p$ with answers and conditions of similar questions retrieved from \database{}. Specifically, the T5 model takes the concatenation of an ambiguous question $q$, a target answer $a$, a passage $p$, and the top $k$ retrieved answers and conditions $\{(a_1, c_1), \dots, (a_k, c_k)\}$ as input to generate the revised question $\tilde{q}$.
\begin{align*}
    \textnormal{input} = &~\textnormal{``question: $q$ + answer $a$ + context: $p$} \\
    &\textnormal{ + hints: $a_1$, $c_1$, ...''}
\end{align*}

\subsubsection{Dataset}
We experiment the question revision task on AmbigQA \cite{min2020ambigqa}. We use the same data that are distantly constructed from evidence articles as in \S \ref{sec:cond_gen}. Again, outputs from models are different -- questions are expected to be revised with contrastive information such that they have unique answers. The constructed dataset contains \hs{num} train and \hs{num} test examples. 



\subsubsection{Results}
\textbf{Baselines} Previous work \cite{min2020ambigqa, gao-etal-2021-answering} simply finetuned a seq-to-seq model, e.g. BART \cite{lewis2020bart}, to predict revised questions. In particular, their input is the concatenation of questions and passages, i.e. ``question: $q$ + answer: $a$ + context: $p$''. This does not provide sufficient information about other answers $\{a_i\}$. Therefore, models are not able to compare answers and find contrastive information to revise questions.

\textbf{Implementation Details} We finetuned a T5-large \cite{raffel2020exploring} model for the question revision task with and without information retrieved from \database{}. In this experiment, we retrieve questions from \database{} and keep a total of 10 answers and conditions from the retrieved questions. Note that some questions have more than one answers. We keep including answers and conditions from top retrieved questions until 10 answers are reached.

\textbf{Main Results} We present the results in Table \ref{tab:ambigqa_result}. In addition to the baseline discussed above (passage-only), we experiment with a few other options that can potentially improve the coverage of information for the revision task. First, we use the question $q$ to retrieve relevant 1 or 2 passages from Wikipedia (wikipedia-1 and wikipedia-2).\footnote{We use JPR \cite{min2021joint} as our passage retriever, same as in \S \ref{sec:asqa_method}.} Retrieved passages should not contain the passage $p$. Second, we expand the passage $p$ with preceding and following tokens to double the length of inputs (passage-expand). Third, we explicitly add a passage $p'$ which contains different answers of the same question (passage-contrast). 

\input{tables_ambigqa_main}

However, none of the proposed alternatives leads to improvement in the question revision task. \hs{check and discuss!!!}

\textbf{Ablations} We run an ablated experiment with different numbers of answers retrieved from \database{}. Without any retrieved answers, the EDIT-F1 is 23.0. As the number of answers increases, the score increases monotonically from 23.0 to 23.8. It shows information from \database{} does help differentiating answers, even though this task is still very challenging to existing models.

\input{tables_ambigqa_abl}





==> 100_model_asqa.tex <==
\section{Experiment: Answer Differentiation with \database{}}
For questions that have different answers, one practical way to answer such questions is to specify under what conditions answers are different from others. For example, in addition to predicting a list of answers, \{``Crisler Center'', ``Michigan Stadium'', ...\}, a QA system should clarify that ``Crisler Center'' is the home stadium of the Michigan basketball team while the ``Michigan Stadium'' is of the football team.

Differentiating answers challenges QA models' ability in multiple ways. First, it requires retrieval models to find diverse information from its source of knowledge such that all answers are present in the retrieved results. Second, the retrieved information should be concise -- longer inputs contain noisy and misleading information and therefore degrade models' performance in differentiating answers. In this experiment, we show that \database{} is a great source of knowledge for the challenging answer differentiation task.  



% retrieving diverse evidence from the corpus and aggregating them to find information that is contrastive.
% For example, ``football'' vs. ``basketball'' is a pair of contrastive information that can differentiate ``Crisler Center'' and ``Michigan Stadium'', while ``men'' vs. ``women'' can not. 


% \section{ASQA}

\subsection{Task}\label{sec:asqa_task}
ASQA is an open-domain question answering (QA) dataset. Different from other open-domain QA datasets, e.g. NQ \cite{kwiatkowski2019natural} and TriviaQA \cite{joshi2017triviaqa}, which requires models to predict only one of the correct answers, ASQA test models' ability to find all correct answers. The expected output for ASQA questions is a short paragraph that summarizes all possible answers as well as clarifying the difference between answers. For example, the expected answer to the question ``Where is the home stadium of the Michigan Wolverines?'' is ``the home stadium of Michigan Wolverines men's football is the Michigan Stadium, while the stadium of its men's basketball team is the Crisler Center. Crisler Center is also the home stadium for Michigan Wolverines women's basketball''.

\subsection{Dataset}
The ASQA dataset contains 4353 train and 948 dev examples. Each example contains an ambiguous question, a list of disambiguated questions and answers (short text spans), and a long-form answer which discusses the difference between short answers. Due to the high variance of long-form answers, each example in ASQA was annotated by two human annotators and the better score among the two annotations is recorded. The average length of answers is 65.0 white-space split tokens. Each question has an average of 3.4 different short answers.


\subsection{Method}\label{sec:asqa_method}
% Similar to the question revision task with AmbigQA (\S \ref{sec:ambigqa_method}), we retrieve a list of similar questions from \database{} and learn a model to summarize their answers and conditions into the long-form answers.
\input{tables_asqa_main}
We use GTR to retrieve top $k$ questions (and the revised questions) from \database{} and apply them for the answer differentiation task. The revised questions provide additional information that are specific to answers. For example, a revised question, ``Where is the home stadium of the Michigan Wolverine men's football in 1997?'', contains several pieces of information \{``men's'', ``football'', ``in 1997''\} for the answer ``Michigan Stadium''. Compared to passages with hundreds of tokens, the revised questions are more concise in capturing relevant information to differentiate answers. 

In addition to questions retrieved from \database{}, we also retrieve a few passages from Wikipedia for generating long-form answers. We find retrieving passages necessary for ASQA, because during annotation it encourages annotators to include background information about the questions in the long-form answers. Such information is not specific to any answer. As a result, merely retrieving from \database{} cannot cover such information required in the output.
% during annotation to make the output more fluent and coherent. Since such background information is not closely relevant to target answers, it is rarely included as conditions in \database{}. 
To mitigate this problem, we follow the baseline to also include top $n$ passages retrieved by JPR \cite{min2021joint} from Wikipedia \cite{stelmakh2022asqa}.\footnote{JPR is an auto-regressive reranking model aiming for increasing the diversity of retrieved passages.}

% \subsubsection{Answer Generation}
Long-form answers are generated from retrieved questions and passages. As discussed above, the generated output should cover multiple answers and discuss the differences between them. We finetune a pretrained T5 model \cite{raffel2020exploring} for the answer generation task. Inputs to the generation model is a concatenation of the original question $q$, answers and conditions of retrieved questions $\{(a_i, c_i)\}$, and retrieved passages $\{p_j\}$.
\begin{align*}
    \textnormal{input} = ~&\textnormal{question: $q$ + conditions: $a_1$, $c_1$, ...}
    \textnormal{ + passages: $p_1$, ...}
\end{align*}

% We finetune a T5 model for answer generation. T5 is finetuned with teacher forcing and makes inference with greedy decoding.

\subsection{Results}
% In the first experiment, we evaluate the recall of the retrieved questions and passages. We varies the number of retrieved questions and passages and check how many answers have been retrieved for the inputs. Like other open-domain QA tasks, recall is an important metric because answers cannot be included to the output if not retrieved. 

% While having more passages can increase the recall, we will show in the second experiment that higher recall may not lead to better answers. We show \hs{add dicussion}.

% \subsubsection{Question Retrieval}
% \textbf{Baseline} We show that \database{} is an efficient way of storing knowledge for multi-answer questions. We compare to the baseline which contains top passages retrieved from Wikipedia. Passages in the baseline are retrieved by JPR \cite{min2021joint} which is an iterative retrieval model designed for increasing the diversity of retrieved answers. JPR shows better coverage of answers for multi-answer questions, compared to other dense retrieval models, such as DPR \cite{karpukhin2020dense}.

% Experimental results are shown in Table \ref{tab:asqa_recall}. As expected, the recall increases as the number of retrieved questions and retrieved passages increases. With as few as 10 answers and 2 passages, the recall becomes comparable to 5 passages (66.1 vs. 66.5), while the total length of the retrieved results is only at 57\% (574.5 vs. 1008.8). With 4 passages plus 10 answers, the length of input decreases by 36.2 (1008.8 to 972.6) while the recall improves from 66.5 to 69.9.

% \input{tables/asqa_recall}
% \hs{TODO: remove duplicated answers}
 

We evaluate the finetuned T5 model on the quality of predicted long-form answers. To show the effectiveness of the retrieved questions and answers from \database{}, we compare to the outputs generated from retrieved passages only. 

Results are presented in Table \ref{tab:asqa_main}. The first group of results (DPR@1 and JPR@1) means we directly return the top 1 passage retrieved by DPR and JPR. The second group of results, e.g. T5 (5 passages), shows the performance of directly generating outputs with the top 5 retrieved passages. Both groups of numbers are copied from the original paper by \citep{stelmakh2022asqa}.

To check whether higher recall from more retrieved passages leads to better outputs, we re-implement the baseline model to run it on more retrieved passages. The results with 5 passages from our implementation matches the numbers reported in the original paper \cite{stelmakh2022asqa}. However, as shown in Table \ref{tab:asqa_main}, as the number of passages increases, both STR-EM and DISAMBIG-F1 drops (40.1 to 39.2, 26.4 to 25.9). 

In the third group of experiments, we retrieve questions from \database{} and add top 10 answers with their conditions to the input. Without changing the model, the performance of long-answer generation with information retrieved from \database{} increases by 0.8 in ROUGE-L and 2.5 in DISAMBIG-F1. In addition, the output length of the model with information from \database{} is also $\sim$10\% shorter than the baseline but covers more answers in its outputs.

\subsection{Ablations} 

\subsubsection{Recall of Answers}
In the first ablation experiment, we justify the claim that retrieving questions from \database{} can improve the diversity of answers. 
We report the recall of answers with and without questions retrieved from \database{} (see Figure \ref{fig:asqa_abl}). 
% Passages in the baseline are retrieved by JPR \cite{min2021joint} which is an iterative retrieval model designed for increasing the diversity of retrieved answers. JPR shows better coverage of answers for multi-answer questions, compared to other dense retrieval models, such as DPR \cite{karpukhin2020dense}. Experimental results are shown in Table \ref{tab:asqa_recall}. 
% As expected, the recall increases as the number of retrieved questions and retrieved passages increases. 
With 10 question and answer pairs from \database{}, the recall of answers improve by around 5 points which leads to around 2 points in the final DR metric.
From another perspective, with as few as 10 answers and 2 passages, the recall becomes comparable to 5 passages (66.1 vs. 66.5). Since information from question and answer pairs are more concise, the total length of 10 answers plus 2 passages is 43\% less (574.5 vs. 1008.8). This concise representation of information eventually leads to 1 point of increase in the final DR metric (34.6 vs. 33.7) as shown in Table \ref{tab:asqa_main}. 

% \input{tables/asqa_recall}
\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{figures_asqa_abl.png}
% \begin{subfigure}{}
% \includegraphics[width=0.4\linewidth]{figures/asqa_qa.png}
% % \caption{Caption 2}
% \label{fig:subim2}
% \end{subfigure}

% \begin{subfigure}{}
% \includegraphics[width=0.4\linewidth]{figures/asqa_qa.png}
% % \caption{Caption 2}
% \label{fig:subim2}
% \end{subfigure}

\caption{\small\label{fig:asqa_abl} Left: Recall of answers from the retrieved results with varying number of passages.  Right: DISAMBIG-F1 of predicted long answers with varying number passages. Both figures show that inputs with more questions yield better outputs under certain number of tokens, in both answer recall and DISAMBIG-F1.}

\end{figure}


\subsubsection{Question Revision}

In the next ablation experiment, we investigate whether the additional information retrieved from \database{} help differentiating answers. Here, we study a question revision sub-task using auxiliary information provided in ASQA.\footnote{This information is also available in the question revision sub-task in AmbigQA \citep{min2020ambigqa}.} 
In this sub-task, the model should revise an ambiguous question using information provided a passage such that it can differentiate the provided answer with others.
% In the first experiment, we would like to use \database{} on a question revision task on AmbigQA \cite{min2020ambigqa}. 
The task is similar to revising questions when constructing \database{} (\S \ref{sec:cond_gen}), except that the additional information added to the revised question should be contrastive, i.e. it should differentiate its answer with others possible answers to the ambiguous questions. For example, to differentiate the answer ``the Michigan Stadium'' and ``Crisler Center'', one should provide the additional information ``\textit{basketball team}'' vs. ``\textit{football team}'', but not ``\textit{built in 1927}'' vs. ``\textit{basketball team}''. 

A naive model simply takes an ambiguous question, an answer, and the provided passage as input to predict the revised question. We instead retrieve similar questions, along with their answers and conditions from \database{}, and augment the provided passage with the retrieved information, similar to \S \ref{sec:asqa_method}. The additional information should provide background knowledge for models to determine how to revise the question. Again, we finetune a T5 model for this question revision task. The model's output is measured by a metric, ``EDIT-F1'', proposed by \citet{min2020ambigqa}, to only evaluate the edits made in the revised questions.\footnote{Please refer to \citet{min2020ambigqa} for more information on ``EDIT-F1''.} 

The results are shown in Table \ref{tab:ambigqa_main}. In addition to the naive baseline of only taking the provided passage as input (passage-only), we experiment with a few other options that can potentially improve the coverage of information for the question revision task. First, we retrieve the top 1 passage from Wikipedia (top-1 Wikipedia).\footnote{We use JPR \cite{min2021joint} as our passage retriever, same as in \S \ref{sec:asqa_method}.} Second, we expand the provided passage with preceding and following tokens to double the length of inputs (passage-expand). Third, we deliberately add a passage which contains different answers of the same question (passage-contrast).\footnote{Also available as auxiliary information in ASQA.} Results in Table \ref{tab:ambigqa_main} shows that adding questions retrieved from \database{} is the most effective method in revising questions, and therefore justify our claim that questions from \database{} are concise and can provide sufficient background information for models to differentiate answers. 

\input{tables_ambigqa_main}



==> 100_model_retrieval.tex <==
\section{Retrieval Using \database{}}
In the first experiment, we evaluate the recall of answers by retrieving from \database{}.
One common problem with existing retrieval models \citep{karpukhin2020dense,ni2021large} in retrieving passages from text corpus for open-domain QA is its lack of diversity of the retrieved results \cite{min2021joint}, i.e. only a subset of answers are obtained from top retrieved passages. This restricts models' performance in predicting multiple answers and further in comparing different answers. We show that we can get more diverse passages by retrieving generated questions from \database{}. %can increase the diversity of answers for multi-answer questions.

\subsection{Method}
We propose to retrieve the most similar questions from \database{} and take the passages where those questions were generated from as the retrievals. Let $x$ be an input question and $p_i$ passages to be retrieved. The score for a passage $p_i$ is
\begin{equation}
    s(x, p_i) = \textnormal{max}_{q'\in \textnormal{GEN}(p)}f(x, q')
\end{equation}
\noindent where $\textnormal{GEN}(p)$ is the set of questions generated from the passage $p$ and $f(x, q')$ is the retrieval score of the question $q' \in \textnormal{GEN}(p)$.
% Retrieving questions from \database{} is analogous to retrieving passages from text corpora. Therefore, 
Any existing retrieval methods can be applied to compute the retrieval score $f(x, q')$. In this experiment, we apply a sparse retrieval model, BM25, and a state-of-the-art dense retrieval model, GTR \citep{ni2021large}. GTR is originally designed for passage retrieval but the query encoder and passage encoder in GTR share their parameters. Therefore, we can directly use it to encode and retrieve questions from \database{}.
We use the checkpoint of GTR finetuned on NQ-open \citep{kwiatkowski2019natural} in our experiment. 
% As discussed above, passages are indirectly retrieved by mapping top-ranked questions to passages where they are generated.  Another simple heuristic to map retrieved questions to passages is to return passages from which the most top-retrieved questions are generated. This method is denoted as (*-count) in Table \ref{tab:ambigqa_retrieval}.\footnote{In the *-count heuristic, we retrieve top 50 questions from \database{} and count which passage generates the most questions out of 50.}

In addition, we propose another simple heuristic to map retrieved questions to passages by returning passages from which the most top-$k$ retrieved questions are generated. We use $k = 50$ in this experiment. 
\begin{equation}
    % s_c(x, p_i) = |\{q' \in \textnormal{GEN}(p_i) ~\textnormal{for}~ q' \in \textnormal{top}_{k}(x)\}|
    s_c(x, p_i) = |\{\textnormal{GEN}(p_i) \cap \textnormal{argmax}_{k, q'}f(x, q')\}|
\end{equation}

\subsection{Dataset}
We use AmbigQA \cite{min2020ambigqa} and WebQuestionsSP \cite{yih-etal-2016-value} in our experiments. AmbigQA is an open-domain QA dataset derived from NQ \cite{kwiatkowski2019natural} which contains questions that are ambiguous and thus have multiple possible answers. WebQuestionsSP (WebQSP) \citep{yih-etal-2016-value} is another dataset which contains open-domain questions asked by web users and a subset of the questions have multiple answers. We only evaluate on multi-answer questions in both datasets in this experiment. 1172 questions in the AmbigQA dev set and 809 questions in the WebQuestionsSP test set have multiple answers.\footnote{We consider questions have multiple answers if at least one of the annotators find multiple answers.}

\subsection{Evaluation} To measure the diversity of retrieval, we evaluate models' performance as the recall of answers. Similar to traditional passage-level retrieval models \citep{karpukhin2020dense}, the recall is measured as the percentage of correct answers that are mentioned in the retrieved passages. 
% However, retrieved candidates from \database{} are questions. To fairly compare with other passage-level retrieval methods, we map the top-ranked questions to passages from which they are generate. The recall of answers is evaluated on the \textit{indirectly} retrieved passages though \database{}.



% Previous methods,, retrieve passages from Wikipedia. Answers are considered as retrieved if they exist in one of the retrieved passages. However, candidates retrieved from \database{} are question and answer pairs. To resolve the mismatch 

% The retrieved passages, commonly with 100 tokens, contains much more information than QA pairs alone from \database{}. To fairly compare with other passage-level retrieval methods, we convert retrieved questions to passages by returning passages from which top-retrieved questions are generated.



% Upon retrieval, we treat the original ambiguous questions as queries, questions in \database{} as keys and answers as values\footnote{Conditions (revised questions) are not used in this task}. We apply one of the dense retrieval models, GTR \cite{ni2021large}, as our retriever to retrieve the top $k$ similar questions from \database{}. GTR is similar to DPR except that GTR's query encoder and passage encoder share same parameters so we can re-use GTR's checkpoint finetuned on NQ \cite{kwiatkowski2019natural} for our question retrieval task. Although GTR is trained for passage retrieval, it is applicable to our task due to its shared encoder. In addition, we also experiment with BM25, a sparse retriever, in the our experiment.


% link retrieved questions in \database{} to the original passages where they are generated, and compute the metrics over the linked passages. 
% We denote this method as (*-top) in Table \ref{tab:ambigqa_retrieval}. Another simple heuristic to return passages from which the most top-retrieved questions are generated. This method is denoted as (*-count) in Table \ref{tab:ambigqa_retrieval}. \footnote{We use the top 50 retrieved questions as the population of relevant questions.}

% Since multiple questions are generated from each passage, questions retrieved from \database{} are likely to be generated from same passages. Having more relevant questions generated from one passage reflects the importance of such passages. To include this heuristic, we propose another method (*-count) which returns passages that generate the most top retrieved questions.

\subsection{Results}
\input{tables_ambigqa_retrieval}

% We compare with passage-level retrieval methods, BM25 and DPR \cite{karpukhin2020dense}. DPR is finetuned on NQ, a superset of questions in AmbigQA.
% \hs{TODO}

Experimental results are presented in Table \ref{tab:ambigqa_retrieval}. Numbers in the first block (passage-based retrieval) show the performance of baseline models, BM25, DPR \citep{karpukhin2020dense} and GTR \citep{ni2021large}, in directly retrieving passages from Wikipedia. DPR is a popular dense retrieval method with separate query and candidate encoders and trained with hard negatives. We re-run the DPR open-sourced code and evaluate the retrieved results. Compared to passage-based retrieval methods, indirect retrieval with \database{} yields better performance in using either BM25 or GTR as the retriever. In particular, the recall@10 with BM25 improves from 44.4 to 45.8 on AmbigQA and from 32.0 to 34.4 on WebQuestionsSP. The performance with GTR is also better with \database{}. On AmbigQA, the recall@10 improves 61.9 to 63.4. More improvement comes on WebQuestionsSP with an increase from 46.3 to 53.0. We conjuecture that the improvement with GTR is less significant on AmbigQA because GTR is pretrained on NQ, which is a super set of questions in AmbigQA.









==> tables_ambigqa_abl.tex <==
\begin{table}[]
\centering
\small
\begin{tabular}{lcccc}
\toprule
\# QA pairs & 0    & 1    & 5    & 10   \\ \midrule
EDIT-F1    & 22.4 & 23.5 & 24.8 & 25.6 \\
\bottomrule
\end{tabular}
\caption{Results on the question revision task of AmbigQA with different numbers of answers and conditions retrieved from \database{}. Results are measured in EDIT-F1. Please refer to \ref{sec:ambigqa_task} for more information on the metrics.}
\label{tab:ambigqa_result}
\end{table}


==> tables_asqa_recall.tex <==
\begin{table}[ht]
\small
\centering
\begin{tabular}{lcccccc}
\toprule
\# psgs & 0     & 1     & 2     & 3     & 4     & 5      \\
\midrule
\multicolumn{7}{l}{\# answers \& conditions: 0}                                  \\
recall    &  --   & 45.3  & 57.1  & 61.6  & 64.4  & 66.5   \\
tokens &  --   & 213.1 & 413.6 & 614.7 & 811.7 & 1008.8 \\
\midrule
\multicolumn{7}{l}{\# answers \& conditions: 5}                                  \\
recall    & 38.3  & 56.7  & 63.8  & 67.0  & 68.1  & 69.8   \\
tokens & 103.2 & 304.7 & 504.0 & 703.4 & 899.9 & 1095.6 \\
\midrule
\multicolumn{7}{l}{\# answers \& conditions: 10}                                 \\
recall    & 44.9  & 60.3  & 66.1  & 68.6  & 69.9  & \textbf{71.1}   \\
tokens & 172.6 & 374.0 & 574.5 & 775.6 & 972.6 & 1169.7 \\
\bottomrule
\end{tabular}
\caption{Recall of answers with different numbers of retrieved questions and passages. Numbers are evaluated on the dev set of ASQA. \hs{Consider making it a figure.}}
\label{tab:asqa_recall}
\end{table}

